A Practical Approach for Computing the Diameter of a Point Set

We present an approximation algorithm for computing the diameter of a point-set in $\Re^d$. The new algorithm is sensitive to the ``hardness'' of computing the diameter of the given input, and for most inputs it is able to compute the exact diameter extremely fast. The new algorithm is simple, robust, has good empirical performance, and can be implemented quickly. As such, it seems to be the algorithm of choice in practice for computing/approximating the diameter.

==> figs/results_mod.tex <==
\begin{table*}[p]
\centerline{
%
\begin{tabular}{|l||r|r|r|r|r|r|r|r|}
    \cline{2-9}
\multicolumn{1}{c||}{}
& \multicolumn{8}{c|}{Running time in seconds}
\\
\hline
  input
& Clock
& Bunny
& Dragon II
& DS9
& Hand
& Dragon
& {\footnotesize Buddha}
& Blade
  \\
  points
&{\footnotesize 30,744}
&{\footnotesize 35,947}
&{\footnotesize 54,831}
&{\footnotesize 298,517}
&{\footnotesize 327,323}
&{\footnotesize 437,645}
&{\footnotesize 543,652}
&{\footnotesize 882,954}
  \\
  \hline%
%
  \hline%
  \multicolumn{1}{|l||}{$\eps=0\Bigl.$}\\
  \hline%
%
FS Heap           & 0.07       & 0.08       & 0.08       & 0.76       & 0.49       & 0.92       & 0.89       & 1.29      \\
FS Heap Ptr & 0.05       & 0.06       & 0.05       & 0.57       & 0.35       & 0.69       & 0.66       & 0.91      \\
FS WSPD           & 0.06       & 0.08       & 0.09       & 0.76       & 0.51       & 0.85       & 0.92       & 1.29      \\
FS Ptr Levels     & 0.06       & 0.08       & 0.09       & 0.63       & 0.41       & 0.83       & 0.79       & 1.18      \\
FS Levels         & 0.07       & 0.09       & 0.11       & 0.80       & 0.52       & 0.94       & 0.99       & 1.52      \\
%
  \hline%
  \hline%
  \multicolumn{1}{|l||}{$\eps=0.01\Bigl.$}\\
  \hline%
%
FS Heap & 0.07       & 0.06       & 0.07       & 0.74       & 0.50       & 0.82       & 0.88       & 1.28      \\
FS Heap Ptr & 0.05       & 0.05       & 0.05       & 0.54       & 0.35       & 0.64       & 0.63       & 0.91      \\
FS WSPD        & 0.06       & 0.06       & 0.07       & 0.74       & 0.48       & 0.79       & 0.87       & 1.27      \\
FS Ptr Levels  & 0.06       & 0.07       & 0.08       & 0.61       & 0.41       & 0.80       & 0.77       & 1.16      \\
FS Levels       & 0.07       & 0.09       & 0.11       & 0.74       & 0.52       & 0.89       & 0.95       & 1.49      \\
Chan           & 0.95       & 1.42       & 1.99       & 3.67       & 6.75       & 9.40       & 11.30      & 12.18     \\
Chan Mod       & 0.87       & 1.25       & 1.83       & 3.55       & 6.60       & 9.27       & 11.23      & 12.05     \\
Grid           & 0.10       & 0.15       & 0.18       & 0.48       & 0.58       & 0.97       & 1.02       & 1.22      \\
FS Directions  & 0.32       & 0.18       & 0.11       & 13.61      & 0.56       & 1.61       & 1.46       & 1.43      \\
%
  \hline%
  \hline%
  \multicolumn{1}{|l||}{$\eps=0.1\Bigl.$}\\
  \hline%
%
FS Heap            & 0.05       & 0.05       & 0.07       & 0.61       & 0.46       & 0.69       & 0.74       & 1.12      \\
FS Heap Ptr & 0.02       & 0.04       & 0.05       & 0.43       & 0.31       & 0.53       & 0.55       & 0.77      \\
FS WSPD         & 0.04       & 0.05       & 0.07       & 0.62       & 0.41       & 0.68       & 0.74       & 1.11      \\
FS Ptr Levels   & 0.04       & 0.06       & 0.07       & 0.50       & 0.36       & 0.61       & 0.62       & 0.90      \\
FS Levels        & 0.05       & 0.07       & 0.10       & 0.62       & 0.47       & 0.71       & 0.78       & 1.17      \\
Chan            & 0.06       & 0.09       & 0.08       & 0.26       & 0.28       & 0.40       & 0.50       & 0.75      \\
Chan Mod        & 0.08       & 0.09       & 0.09       & 0.27       & 0.30       & 0.41       & 0.51       & 0.74      \\
Grid            & 0.03       & 0.04       & 0.05       & 0.25       & 0.26       & 0.36       & 0.43       & 0.68      \\
Grid FS Dir     & 0.04       & 0.03       & 0.05       & 0.25       & 0.25       & 0.35       & 0.42       & 0.69      \\
FS Directions   & 0.09       & 0.06       & 0.08       & 1.58       & 0.45       & 0.75       & 0.82       & 1.11      \\
%
  \hline%
  \multicolumn{2}{|c|}{$\eps=\frac{\sqrt{3}-1}{\sqrt{3}} \approx 0.73\Bigr.$}\\
  \hline%
%
BBox           & 0.00       & 0.01       & 0.00       & 0.03       & 0.03       & 0.05       & 0.07       & 0.10      \\
PCA            & 0.01       & 0.01       & 0.02       & 0.08       & 0.08       & 0.12       & 0.14       & 0.22      \\

%
%
%
%
%
%
%
%
%
%
%
\hline
%
\end{tabular}}
\caption{Results for various models}
\label{tbl:results:mod}
\end{table*}

%
%
%
%


==> figs/results_syn.tex <==
\begin{table*}[p]
%
    \centerline{
\begin{tabular}{|l||r|r|r|r||r|r|r|r|}
    %
    \cline{2-9}
\multicolumn{1}{c||}{}
& \multicolumn{8}{c|}{Running time in seconds}
\\
\cline{2-9}
  \multicolumn{1}{c||}{}
& \multicolumn{4}{c||}{Sphere}
& \multicolumn{4}{c|}{ARCS}
\\
\hline
  input
&  $10^3$
&  $10^4$
&  $10^5$
&  $10^6$
&  $10^3$
&  $10^4$
&  $10^5$
&  $2*10^5$\\
points                & 1,000      & 10,000     & 100,000    & 200,000    & 1,000      & 10,000     & 100,000    & 200,000   \\
%
  \hline%
  \multicolumn{1}{|l||}{$\eps=0$}\\
  \hline%
%
  FS Heap           & 0.04       & 1.14       & 50.15      & 202.26     & 0.03       & 0.01       & 0.04       & 0.08      \\
FS Heap Ptr & 0.03       & 2.47       & 144.63     & 450.29     & 0.04       & 0.00       & 0.03       & 0.07      \\
FS WSPD           & 0.04       & 1.19       & 53.74      & 157.08     & 0.03       & 0.00       & 0.05       & 0.09      \\
FS Ptr Levels     & 0.03       & 1.00       & 49.55      & 179.26     & 0.03       & 0.00       & 0.04       & 0.08      \\
FS Levels         & 0.03       & 1.05       & 52.02      & 186.01     & 0.03       & 0.01       & 0.06       & 0.11      \\
%
  \hline%
  \multicolumn{1}{|l||}{$\eps=0.01$}\\
  \hline%
%
FS Heap & 0.07       & 0.96       & 34.32      & 140.69     & 0.06       & 0.00       & 0.03       & 0.09      \\
FS Heap Ptr & 0.06       & 2.11       & 126.57     & 371.62     & 0.07       & 0.00       & 0.03       & 0.08      \\
FS WSPD        & 0.03       & 1.00       & 37.12      & 96.99      & 0.00       & 0.01       & 0.05       & 0.09      \\
FS Ptr Levels  & 0.03       & 0.82       & 33.85      & 122.99     & 0.00       & 0.00       & 0.05       & 0.09      \\
FS Levels       & 0.04       & 0.88       & 35.62      & 130.08     & 0.00       & 0.01       & 0.06       & 0.10      \\
Chan           & 0.04       & 0.50       & 3.48       & 6.45       & 0.00       & 0.06       & 0.13       & 0.20      \\
Chan Mod       & 0.03       & 0.81       & 3.82       & 6.96       & 0.00       & 0.07       & 0.13       & 0.20      \\
Grid           & 0.21       & 0.99       & 39.68      & 125.04     & 0.06       & 0.03       & 0.10       & 0.16      \\
FS Directions  & 0.33       & 1.41       & 440.65     & 961.95     & 0.06       & 0.01       & 0.05       & 0.10      \\
%
  \hline%
  \multicolumn{1}{|l||}{$\eps=0.1$}\\
  \hline%
%
FS Heap            & 0.05       & 0.15       & 0.35       & 0.70       & 0.02       & 0.00       & 0.05       & 0.10      \\
FS Heap Ptr & 0.03       & 0.42       & 5.17       & 6.21       & 0.00       & 0.00       & 0.03       & 0.07      \\
FS WSPD         & 0.02       & 0.18       & 0.33       & 0.64       & 0.00       & 0.00       & 0.05       & 0.09      \\
FS Ptr Levels   & 0.02       & 0.12       & 0.35       & 0.74       & 0.00       & 0.01       & 0.04       & 0.08      \\
FS Levels        & 0.02       & 0.13       & 0.32       & 0.67       & 0.00       & 0.00       & 0.05       & 0.11      \\
Chan            & 0.02       & 0.07       & 0.17       & 0.26       & 0.00       & 0.01       & 0.07       & 0.16      \\
Chan Mod        & 0.02       & 0.06       & 0.17       & 0.26       & 0.00       & 0.01       & 0.07       & 0.15      \\
Grid            & 0.01       & 0.16       & 0.26       & 0.34       & 0.00       & 0.01       & 0.08       & 0.15      \\
Grid FS Dir     & 0.01       & 0.29       & 0.40       & 0.49       & 0.00       & 0.00       & 0.07       & 0.15      \\
FS Directions   & 0.03       & 0.46       & 8.16       & 16.72      & 0.00       & 0.01       & 0.04       & 0.09      \\
%
  \hline%
  \multicolumn{1}{|l||}{$\eps=\frac{\sqrt{3}-1}{\sqrt{3}} \approx 0.73$}\\
  \hline%
%
BBox           & 0.02       & 0.00       & 0.01       & 0.02       & 0.00       & 0.00       & 0.02       & 0.02      \\
PCA            & 0.02       & 0.00       & 0.03       & 0.05       & 0.00       & 0.01       & 0.02       & 0.05      \\

%
%
%
%
%
%
%
%
%
%
%
\hline
\end{tabular}
}
\caption{Results for syntetic inputs}
\label{tbl:results:syn}
\end{table*}

%
%
%
%


